Detector Response Matrices, Effective Areas, and Flash-Effective Areas for Radiation Detectors

A Detector Response Matrix (DRM) is a discrete representation of an instrument's Detector Response Function (DRF), which quantifies how many discrete energy depositions occur in a detector volume for a given distribution of particles incident on the detector. For simple radiation detectors that can count such energy depositions (such as scintillators, Proportional Counter Tubes (PCTs), etc), we consider the ideal counting DRF, $\mathbf{G}_\varphi (E_\mathrm{in}, E_\mathrm{dep})$, which relates the detector's counting histogram (number of energy depositions within a given channel) to an incident particles characterization, $\varphi$ (e.g. incident flux, fluence, intensity). From the counting DRF we can derive the counting DRM, the effective area, and the flash effective area (which measures the total energy deposited in the detector from a large, instantaneous fluence).

==> commands.tex <==
\newlength\sqsz
\sqsz=1.4cm
\newcommand\sq[2][white]{\protect\sqhelper{#1}{#2}{}}
\newcommand\sqhelper[2]{\sffamily\bfseries\fboxsep=-\fboxrule%
  \def\sqcolor{#1}\def\sqcat{low}%
  \fcolorbox{black}{\sqcolor}{\makebox[\sqsz]{%
  \rule[\dimexpr-.5\sqsz+.2\ht\strutbox]{0pt}{\sqsz}#2}}}
  %\rule[\dimexpr-.5\sqsz+.2\ht\strutbox]{0pt}{\sqsz}\stackanchor[2pt]{#1}{}}}}
\newcommand\hsq[1]{\protect\hsqhelper{#1}}
\newcommand\hsqhelper[1]{\sffamily\bfseries%
  \makebox[\sqsz]{\rule{0pt}{\dimexpr.5\sqsz+.2\ht\strutbox}#1}}
\newcommand\vsq[1]{\protect\vsqhelper{#1}}
\newcommand\vsqhelper[1]{\sffamily\bfseries%
  \rule[\dimexpr-.5\sqsz+.2\ht\strutbox]{0pt}{\sqsz}#1}


\newcommand{\bal}[1]{\textcolor{orange}{[BAL: #1]}}
%\newdate{\today}

\newcommand{\EdepSum}{\sum_{\substack{j \in \\ E_A < E_\mathrm{dep}^{(j)}<{E_B}}}}


%create command for markings on top and bottom of page
%change font size/color/etc here to maintain consistency
\newcommand\topMarkings[1]{%
\renewcommand\@topMarkings{\markingfont#1}%
}
\newcommand\@topMarkings{}

\newcommand\bottomMarkings[1]{%
\renewcommand\@bottomMarkings{\markingfont#1}%
}
\newcommand\@bottomMarkings{}

\newcommand\markings[1]{%
\topMarkings{\markingfont#1}
\bottomMarkings{\markingfont#1}
%\renewcommand\@markings{\markingfont#1}%
}
\newcommand\@markings{}


%redefine \section to save section title for putting in header and resets page number to 1
\newcommand\appendixmode[1]{%
\renewcommand\@appendixmode{#1}%
}
\newcommand\@appendixmode{}

\newcommand\appendixSections[1]{%
\if\relax\noexpand#1\relax
\appendixmode{}
\else 
\appendixmode{1}
\fi
}

\newcommand\sectiontitle{}
\newcommand\subsectiontitle{}
\newcommand\subsubsectiontitle{}
\let\oldsection\section
\let\oldsubsection\subsection
\let\oldsubsubsection\subsubsection
\let\oldpage\thepage

\newcounter{@secnumdepth}

\usepackage{titletoc}

\RenewDocumentCommand{\section}{s o m}{%
\FloatBarrier  
    \setcounter{figure}{0}\setcounter{table}{0}%\setcounter{tocdepth}{0}
  \IfBooleanTF{#1}
    {\setcounter{@secnumdepth}{\value{secnumdepth}}% Store secnumdepth
     \setcounter{secnumdepth}{0}% Print only up to \chapter numbers
     {\thispagestyle{markings}}\setcounter{page}{1}\oldsection{#3}\renewcommand{\sectiontitle}{#3}% \section*
     \setcounter{secnumdepth}{\value{@secnumdepth}} }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {{\thispagestyle{markings}}\setcounter{page}{1}\oldsection[#2]{#3}\renewcommand{\sectiontitle}{#3}}% \section[.]{..}
       {{\thispagestyle{markings}\thispagestyle{contents}}\setcounter{page}{1}\oldsection{#3}\renewcommand{\sectiontitle}{#3}}}%
       \pagestyle{contents}% \section{..}
 \renewcommand{\thepage}{\thesection-\arabic{page}}\renewcommand\thefigure{\thesection-\arabic{figure}}\renewcommand\thetable{\thesection-\arabic{table}} %\label{#3}%
\FloatBarrier%

       %\addtocontents{toc}{\contentsline{section}{\numberline{\thesection}\sectiontitle}{\thesection-\thepage}}

}



\RenewDocumentCommand{\subsection}{s o m}{%
\FloatBarrier 
\IfBooleanTF{#1}
{\oldsubsection*{#3}}
{\IfValueTF{#2}% \section
    {\oldsubsection[#2]{#3}}
    {\oldsubsection{#3}}
    }
\FloatBarrier
}%

\RenewDocumentCommand{\subsubsection}{s o m}{%
\FloatBarrier 
\IfBooleanTF{#1}
{\oldsubsubsection*{#3}}
{\IfValueTF{#2}% \section
    {\oldsubsubsection[#2]{#3}}
    {\oldsubsubsection{#3}}
    }
\FloatBarrier
}%


%create new variable to store start page number for executive summary
%used to prevent section title from being in header on first page
%avoid using \renewcommand, as \executivepage will update with \thepage, rather than keeping its original value


\NewDocumentCommand{\frontmattersection}{s o m}{%
\FloatBarrier\setcounter{figure}{0}\setcounter{table}{0}%
  \IfBooleanTF{#1}
    {\setcounter{@secnumdepth}{\value{secnumdepth}}% Store secnumdepth
     \setcounter{secnumdepth}{0}% Print only up to \chapter numbers
     \clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection{#3}\renewcommand{\sectiontitle}{#3}% \section*
     \setcounter{secnumdepth}{\value{@secnumdepth}} }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection[#2]{#3}\renewcommand{\sectiontitle}{#3}}% \section[.]{..}
       {\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection{#3}\renewcommand{\sectiontitle}{#3}}}%
       \pagestyle{frontmatter}% 
       \renewcommand{\thepage}{\roman{page}}%
       \edef\startPage{\thepage}%\section{..}%
        \label{#3}\FloatBarrier%
        
}






\newcounter{@appendixnumber}
\setcounter{@appendixnumber}{0}
\NewDocumentCommand{\appendixsection}{s o m}{%
\FloatBarrier
  \setcounter{figure}{0}
  \setcounter{table}{0}
   \setcounter{subsection}{0}


     \clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{appendix}}\stepcounter{@appendixnumber}\setcounter{page}{1}\renewcommand{\sectiontitle}{Appendix\hspace{2pt}\Alph{@appendixnumber}:\hspace{4pt}#3}\titleformat{\section}{\heading\selectfont}{}{0pt}{}[]\renewcommand{\thesection}{\Alph{@appendixnumber}}\phantomsection\oldsection*{\sectiontitle}%% \section*
    \stepcounter{section}
    \pagestyle{appendix}% \section{..}
       
    \renewcommand{\thepage}{\Alph{@appendixnumber}-\arabic{page}}\renewcommand\thefigure{\Alph{@appendixnumber}-\arabic{figure}}\renewcommand\thetable{\Alph{@appendixnumber}-\arabic{table}}\label{#3}\FloatBarrier%
    
    %add TOC entry.  Allow TOC name to be passed with [] option when section is created
    \IfValueTF{#2}%
    {\addcontentsline{toc}{section}{Appendix\hspace{2pt}\Alph{@appendixnumber}:\hspace{4pt}#2}}
    {\addcontentsline{toc}{section}{\sectiontitle}}
}%
  


\NewDocumentCommand{\appendixsubsection}{s o m}{%
\FloatBarrier
\setcounter{subsubsection}{0}
  \IfBooleanTF{#1}
    {
     \renewcommand{\subsectiontitle}{#3}\oldsubsection{#3}% \section*
      }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\renewcommand{\subsectiontitle}{#3}}\oldsubsection[#2]{\subsectiontitle}% \section[.]{..}
       {\oldsubsection{#3}\renewcommand{\subsectiontitle}{#3}}}%
       \titleformat{\subsection}{\subheading\selectfont}{}{0pt}{}[]%
    \FloatBarrier
}%

\NewDocumentCommand{\appendixsubsubsection}{s o m}{%

\FloatBarrier
  \IfBooleanTF{#1}
    {
     \renewcommand{\subsubsectiontitle}{#3}\oldsubsubsection{#3}% \section*
      }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\renewcommand{\subsubsectiontitle}{#3}}\oldsubsubsection[#2]{\subsubsectiontitle}% \section[.]{..}
       {\oldsubsubsection{#3}\renewcommand{\subsubsectiontitle}{#3}}}%
       \titleformat{\subsubsection}{\subsubheading\selectfont}{}{0pt}{}[]%
     \FloatBarrier
}%



\let\oldprintbibliography\printbibliography%
\newcommand{\ShowBibliography}[0]{%
\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{contents}}%

\thispagestyle{contents}%
\setcounter{@appendixnumber}{18}%
\renewcommand{\sectiontitle}{References}%
\renewcommand{\thepage}{R-\oldpage}%
%print heading then change page style contents, then print biblio without heading
%needed otherwise first page will have wrong page style
\printbibheading
\thispagestyle{contents}
\pagestyle{contents}
\oldprintbibliography[heading=none]


\renewcommand{\thepage}{R-\oldpage}%
}%

\begin{comment}
\RenewDocumentCommand{\printbibliography}{s o m}{%
%{\clearpage{\thispagestyle{markings}\cleardoublepage}%
%}%
%\thispagestyle{contents}
%\setcounter{@appendixnumber}{18}
%\renewcommand{\sectiontitle}{References}
\oldprintbibliography
%\thispagestyle{contents}
%
%\renewcommand{\thepage}{R-\oldpage}%
}%




\let\oldprintbibliography\printbibliography
\RenewDocumentCommand{\printbibliography}{s o m}{%
\oldprintbibliography%
\renewcommand{\sectiontitle}{References}
%\thispagestyle{references}%
\renewcommand{\thepage}{R-\oldpage}%
}
\end{comment}

%Redefine TOC so page doesn't reset and it keeps the right pagestyle
\let\oldtableofcontents\tableofcontents
\renewcommand{\tableofcontents}{%
   \pagestyle{markings} \cleardoublepage \pagestyle{contents}
   \edef\startPage{\thepage}
   
\tocloftpagestyle{contents}
\renewcommand{\sectiontitle}{Contents}
\let\oldoldsection\section
\renewcommand{\section}{\oldsection}
\renewcommand{\thepage}{\roman{page}}
\renewcommand{\cftsecleader}{\cftdotfill{\cftdotsep}}


%make a TOC
\oldtableofcontents

%set so up to subsubsections are shown in TOC
\setcounter{tocdepth}{3}

%disable \clearpage so list of figure and tables don't create a new page and are listed directly after TOC
\let\LaTeXStandardClearpage\clearpage
\let\clearpage\relax
  % Do nothing when a \clearpage command appears 
\renewcommand{\listfigurename}{Figures}
\listoffigures
\pagestyle{frontmatter}
\renewcommand{\listtablename}{Tables}
\listoftables
\let\clearpage\LaTeXStandardClearpage % Return to the old definition


%reset section definition 
\let\section\oldoldsection


}



==> fonts.tex <==
%%%%%%%%%%Set Caption Font%%%%%%%%%
\usepackage{caption}
\DeclareCaptionFont{caption}{\sourcesanspro\captiongrey\fontsize{9}{12}\selectfont}
\usepackage[font=caption]{caption}



%%%%%%%%%%%LANL colors%%%%%%%%%%%%%
\newcommand{\primarycolor}{\color[HTML]{000F7E}}
\newcommand{\primarygradient}{\color[HTML]{090238}}
\newcommand{\secondarycolor}{\color[HTML]{0070C1}}
\newcommand{\secondarycolortwo}{\color[HTML]{3296DC}}
\newcommand{\secondarycolorthree}{\color[HTML]{69C3FF}}
\newcommand{\captiongrey}{\color[HTML]{555962}}


%%%%%%%%%%%%Fonts%%%%%%%%%%%%%%%%%%%%
%fonts from style guide note: acumin not avaialable in latex, using URW Grotesk
%acumin used for heading, source sans pro used for body, captions, etc.
\newcommand{\acumin}{\fontfamily{ugq}}
\newcommand{\sourcesanspro}{\fontfamily{SourceSansPro-TLF}}

%font types listed in style guide
\newcommand{\fontone}{\acumin \fontsize{38}{40}\fontseries{bx}}
\newcommand{\fonttwo}{\acumin \fontsize{24}{28}\fontseries{b}}
\newcommand{\fontthree}{\sourcesanspro \fontsize{15}{22}\fontseries{b}}
\newcommand{\fontfour}{\sourcesanspro \fontsize{10}{14}\fontseries{sb}}
\newcommand{\fontfive}{\sourcesanspro \fontsize{10}{14}}

%define fonts for headings in Word report template
\newcommand{\headingfont}{\normalfont \fontsize{14}{18}\fontseries{bx}}
\newcommand{\subheadingfont}{\normalfont \fontsize{12}{16}\fontseries{b}}
\newcommand{\subsubheadingfont}{\normalfont \fontsize{11}{15}\fontshape{it}}

%define fonts+color for use in headings
\newcommand{\heading}{\headingfont\primarycolor}
\newcommand{\subheading}{\subheadingfont\primarycolor}
\newcommand{\subsubheading}{\subsubheadingfont\primarycolor}


\newcommand{\tableheading}{\acumin\fontseries{bx}\fontsize{11}{12}\selectfont}
\newcommand{\markingfont}{\sourcesanspro\fontsize{14}{0}\fontseries{bx}\selectfont}
\newcommand{\OUOfont}{\markingfont}
\newcommand{\CUIfont}{\markingfont}
\newcommand{\ClassfiedFont}{\color{red}\markingfont}

\newcommand{\SRD}{\color{red}\markingfont SECRET//RESTRICTED DATA}
\newcommand{\OUO}{\OUOfont Official Use Only}
\newcommand{\CUI}{\CUIfont \@CUIcategory}
\newcommand{\ECI}{\OUOfont Export Controlled Information}
%\newcommand{\markingfont}{\acumin\color{red}\fontsize{20}{0}\fontseries{bx}\selectfont}
%\newcommand{\captionfont}{\sourcesanspro\fontsize{9}{12}\selectfont}
%define section headers as shown in word template



%add [runin] after {\section} if you don't want new line after header
%{xxpt} controls distance between section number and section title
\titleformat{\section}{\heading\selectfont}{\thesection}{10pt}{}[]
\titleformat{\subsection}{\subheading\selectfont}{\thesubsection}{10pt}{}[]
\titleformat{\subsubsection}{\subsubheading\selectfont}{\thesubsubsection}{10pt}{}[]


==> pagestyles.tex <==
%%%%%%%%%%%%page styles%%%%%%%%%%%
%Generic markings page
\fancypagestyle{markings}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[C]{ \vspace{30pt}  \@bottomMarkings } \fancyhead[C]{\@topMarkings } }

%Exectuive Summary page style
\fancypagestyle{frontmatter}{  \fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont\sectiontitle }


%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ 
\ifthenelse{\equal{\thepage}{\startPage}}{}{\heading\selectfont\sectiontitle}
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
    \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }% 
}

\fancypagestyle{}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[C]{ \@bottomMarkings } \fancyhead[C]{\@topMarkings}}



%Title page, includes markings and LANL logo in bottom left of footer
\fancypagestyle{title}{\pagenumbering{roman}\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[L]{\hspace*{-0.5in}\begin{tikzpicture}
  \node[opacity=0.5,inner sep=0pt] at (0,0)
   {\includegraphics[scale=.75]{LANL_Logo_Ultramarine.png}};
  \end{tikzpicture} \leavevmode  \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}} \fancyhead[C]{\@topMarkings}}
  
  
%Preparation page, has LANL logo and disclaimer with markings below 
 \fancypagestyle{preparation}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[L]{\begin{tikzpicture}
  \node[opacity=0.5,inner sep=0pt] at (0,0)
   {\includegraphics[scale=.75]{LANL_Logo_Ultramarine.png}};
  \end{tikzpicture} \leavevmode \\ 
\fontsize{8}{10}\selectfont\noindent Los Alamos National Laboratory, an affirmative action/equal opportunity employer, is managed by Triad National Security, LLC, for the National Nuclear Security Administration of the U.S. Department of Energy, under contract 89233218CNA000001. By acceptance of this article, the publisher recognizes that the U.S. Government retains a nonexclusive, royalty-free license to publish or reproduce the published form of this contribution, or to allow others to do so, for U.S. Government purposes. Los Alamos National Laboratory requests that the publisher identify this article as work performed under the auspices of the U.S. Department of Energy. Los Alamos National Laboratory strongly supports academic freedom and a researcher’s right to publish; as an institution, however, the Laboratory does not endorse the viewpoint of a publication or guarantee its technical correctness.
  \leavevmode \\
  \begin{center}\vspace{15pt}\@bottomMarkings\end{center}} 
  
  
  \fancyhead[C]{\@topMarkings}}

%Contents pages, includes centered markings and section header on the left/right for even/odd pages
\fancypagestyle{contents}{%

%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center}\heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center}  \leavevmode \\ \ifthenelse{\equal{\value{page}}{1}}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
    \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }%
}


%references pages, includes centered markings and section header on the left/right for even/odd pages
\fancypagestyle{references}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center}\heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center}  \leavevmode \\ \ifthenelse{\equal{\value{page}}{1}}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
    \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage\leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }%


}


\fancypagestyle{appendix}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}


\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ \ifthenelse{\oldpage=1}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
    \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage  \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }%
}

\fancypagestyle{references}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}


\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont References }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ \ifthenelse{\thepage=1}{}{\heading\selectfont References}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad R-\thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
    \raggedright Los Alamos National Laboratory \hfill Page\quad R-\thepage \leavevmode 
        \begin{center}\vspace{-6pt}\@bottomMarkings\end{center}
    }%
}


